The puzzling origin of the 6Li plateau

We discuss the 6Li abundance evolution within a hierarchical model of Galaxy formation which correctly reproduces the [Fe/H] distribution of metal-poor halo stars. Contrary to previous findings, we find that neither the level (6Li/H=6x10^-12) nor the flatness of the 6Li distribution with [Fe/H] can be reproduced under the most favourable conditions by any model in which 6Li production is tied to a (data-constrained) Galactic star formation rate via cosmic ray spallation. Thus, the origin of the plateau might be due to some other early mechanism unrelated to star formation.

==> Makefile <==
#
# Makefile for LaTeX
# Version: 2007-11-22
#

### file
TARGET = lithium_main
INPUTS = lithium_preamble.tex lithium_main.tex lithium_introduction.tex lithium_model.tex lithium_results.tex lithium_discussion.tex
VPATH = source_tex 

### programs
LATEX  = latex
BIBTEX = bibtex
DVIPS  = dvips
DVIPDF = dvipdf

### targets
$(TARGET).dvi: $(TARGET).tex $(TARGET).bbl $(INPUTS)
	$(LATEX)  $(TARGET) 
	$(LATEX)  $(TARGET)

$(TARGET).bbl: $(TARGET).bib
	$(LATEX) $(TARGET)
	$(BIBTEX) $(TARGET)

ps: $(TARGET).ps

pdf: $(TARGET).pdf

### clean up
clean:
	find . -maxdepth 1 -name $(TARGET).log -exec rm {} \;
	find . -maxdepth 1 -name $(TARGET).aux -exec rm {} \;
	find . -maxdepth 1 -name $(TARGET).toc -exec rm {} \;
	find . -maxdepth 1 -name $(TARGET).lof -exec rm {} \;
	find . -maxdepth 1 -name $(TARGET).lot -exec rm {} \;
	find . -maxdepth 1 -name $(TARGET).bbl -exec rm {} \;
	find . -maxdepth 1 -name $(TARGET).blg -exec rm {} \;
	find . -maxdepth 1 -name *.bib~ -exec rm {} \;
	find . -maxdepth 2 -name *.tex~ -exec rm {} \;

clean-dvi:
	find . -maxdepth 1 -name $(TARGET).dvi -exec rm {} \;

clean-ps:
	find . -maxdepth 1 -name $(TARGET).ps -exec rm {} \;

clean-all: clean clean-dvi clean-ps

### implicit rules
.dvi.ps:
	$(DVIPS) $< -o $@

.dvi.pdf:
	$(DVIPDF) $< $@

### tar all
#$(latexfile).tar.gz : $(figures) $(latexfile).tex
#        tar -czvf $(latexfile).tar.gz $(figures) $(latexfile).tex Figs/*.fig
#tarball: $(latexfile).tar.gz

### misc
.SUFFIXES: .tex .aux .toc .lof .lot .log .dvi .ps .pdf

#
# EOF
#

